Provable Guarantees for Self-Supervised Deep Learning with Spectral Contrastive Loss

Recent works in self-supervised learning have advanced the state-of-the-art by relying on the contrastive learning paradigm, which learns representations by pushing positive pairs, or similar examples from the same class, closer together while keeping negative pairs far apart. Despite the empirical successes, theoretical foundations are limited -- prior analyses assume conditional independence of the positive pairs given the same class label, but recent empirical applications use heavily correlated positive pairs (i.e., data augmentations of the same image). Our work analyzes contrastive learning without assuming conditional independence of positive pairs using a novel concept of the augmentation graph on data. Edges in this graph connect augmentations of the same data, and ground-truth classes naturally form connected sub-graphs. We propose a loss that performs spectral decomposition on the population augmentation graph and can be succinctly written as a contrastive learning objective on neural net representations. Minimizing this objective leads to features with provable accuracy guarantees under linear probe evaluation. By standard generalization bounds, these accuracy guarantees also hold when minimizing the training contrastive loss. Empirically, the features learned by our objective can match or outperform several strong baselines on benchmark vision datasets. In all, this work provides the first provable analysis for contrastive learning where guarantees for linear probe evaluation can apply to realistic empirical settings.

==> proof_example_archive.tex <==
\section{Proofs for Section~\ref{section:gaussian_example}}\label{section:proof_of_gaussian_example}
In this section we give a proof of Theorem~\ref{theorem:gaussian_example}. 

%We first define the following property that captures our assumption on the transformation functions.
%\begin{definition}[$(\gamma, \eta)$-discrete function]
%	We say a function $\augexample: \Real^d\rightarrow \img$ is a $(\gamma, \eta)$-discrete function with image $\img$ if: $\img$ is a finite set and for any two data $x, x'\in\Real^d$ such that $\norm{x}_2\le\gamma$, $\norm{x'}_2\le\gamma$ and $\norm{x-x'}_2>\eta$, there is $\augexample(x)\ne \augexample(x')$.
%\end{definition}

%We note that the assumptions of $\augexample_i$ in Theorem~\ref{theorem:gaussian_example} essentially means every $\augexample_1$ is a $(\gamma, \eta)$-discrete function with some $\gamma \ge $
The following lemma shows that the augmented graph for Example~\ref{example:gaussian} satisfies Assumption~\ref{definition:accurate_partition} with some bounded $\alpha$.

\begin{lemma}\label{lemma:gaussian_example_lemma1}
	In the setting of Theorem~\ref{theorem:gaussian_example}, assume for any $x, x'\in\Real^d$ such that $\|{x}\|_2+ \|{x'}\|_2\le 2 \max_i\|{\mu_i}\|_2$ and $\|{x-x'}\|_2> \frac{1}{10} \min_{i\ne j}\|{\mu_i-\mu_j}\|_2$, there is $\augexample_t(x)\ne \augexample_t(x')$ for any $t\in[m]$. Then, the data distribution satisfies Assumption~\ref{definition:accurate_partition} with
	\begin{align*}
	\alpha :=1-\Phi_{d}\left(\frac{\Delta_\mu}{5}\right)\cdot \Phi_{d}\left(\frac{\Delta_\mu}{5\sigma}\right),
	\end{align*}
	where $\Phi_{d}(z) := \Pr_{\xi\sim\mathcal{N}(0, I)} (\norm{\xi}_2\le z)$ and $\Delta_\mu := \min_{i\ne j} \norm{\mu_i - \mu_j}_2$.
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{lemma:gaussian_example_lemma1}]
	Let $\img=\cup_{i\in[m]}\img_i$ where $\img_i$ is the image of function $\augexample_i$. We define function $\hat{y}: \img \rightarrow[r]$ as follows. For any ${x}\in \img$, assuming ${x}\in \img_i$, we let $\hat{y}({x}) := j$ if there exists some $j$ such that $y(x')=j$ for $\forall x'\in \augexample_i^{-1}({x})$. If no such $j$ exists, we let $\hat{y}({x}):=1$.
	
	%	
	%	Since the bijection functions have disjoint images, we can define function 
	%	\begin{align}
	%	\hat{y}(x) = \sum_{i=1}^B y(A_i^{-1}(x)) \id{x\in A_i[\Real^d]}.
	%	\end{align} 
	%	There is 
	%	\begin{align}
	%	\phi^{\hat{y}} &= \Exp{x\sim \pndata} \left[\Pr_{x'\sim \aug{x}, x''\sim \aug{x}}(\hat{y}(x')\ne \hat{y}(x'')) \right]\\
	%	&= \Exp{x\sim \pndata} \left[ \Pr_{\epsilon_1\sim \mathcal{N}(0, \sigma^2), \epsilon_2\sim \mathcal{N}(0, \sigma^2)} (y(x+\epsilon_1) \ne y(x+\epsilon_2))\right]\\
	%	&\le 1-\Phi_{d}\left(\frac{\Delta_\mu}{4}\right) \cdot \Phi_d\left(\frac{\Delta_\mu}{4\sigma}\right)^2.
	%	\end{align}
	%	Here the inequality is because when $\norm{x-\mu_i}\le \frac{\Delta_\mu}{4}$ for some $\mu_i$, $\norm{\epsilon_1}\le \frac{\Delta_\mu}{4} $ and $\norm{\epsilon_2}\le \frac{\Delta_\mu}{4} $, there has to be $y(x+\epsilon_1) = y(x+\epsilon_2)$.
	
	When some $x\in\Real^d$ and $\xi\in\Real^d$ satisfy $\norm{x-\mu_i}_2\le \frac{\Delta_\mu}{5}$ for some $\mu_i$ and $\norm{\xi}_2\le \frac{\Delta_\mu}{5}$, there must be for any $x'$ such that $\norm{x'-(x+\xi)}_2\le\Delta_\mu/10$, there is
	$
	\norm{x'}_2\le 2\max_{i}\norm{\mu_i}_2
	$
	and 
	$
	y(x')=y(x+\xi) = y(x)
	$.
	By the assumption of $\augexample_i$ and the definition of $\hat{y}$, there is $\hat{y}(\augexample_i(x+\xi)) = y(x)$ for all $i\in[m]$.
	Therefore, we have
	\begin{align*}
	\Pr_{\bar{x}\sim\pndata, {x}\sim\aug{\bar{x}}}(\hat{y}({x})\ne y(\bar{x})) 
	\le 1-\Phi_{d}\left(\frac{\Delta_\mu}{5}\right)\cdot \Phi_{d}\left(\frac{\Delta_\mu}{5\sigma}\right) =\alpha.
	\end{align*}
%	So the partition induced by $\hat{y}$ is an $\alpha$-accurate partition of graph $G$.	
\end{proof}

We use the following lemma to give a lower bound for the sparest $m$-partition of the augmentation graph in Example~\ref{example:gaussian}.

\begin{lemma}\label{lemma:gaussian_example_lemma2}
	In the setting of Theorem~\ref{theorem:gaussian_example}, for any $k'>r$ and $\tau>0$, there is 
	\begin{align*}
	\rho_{k'} \ge \frac{c_\tau}{18} \cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right),
	\end{align*}
	where $c_\sigma := \sigma \cdot  \Phi_d^{-1}(\frac{2}{3})$
	with $\Phi_{d}(z) := \Pr_{\xi\sim\mathcal{N}(0, I)} (\norm{\xi}_2\le z)$, and
	$
	c_\tau  := \min_{p \in[0, \frac{3}{4}]} \frac{\Phi(\Phi^{-1}(p)+\tau)}{p} - 1
	$
	with 
	$
	\Phi(z) := \int_{-\infty}^z  \frac{e^{-u^2/2}}{\sqrt{2\pi}}du.
	$
\end{lemma}

The proof of Lemma~\ref{lemma:gaussian_example_lemma2} can be found in Section~\ref{section:proof_of_gaussian_lemma2}. Now we give the proof of Theorem~\ref{theorem:gaussian_example} by combining Lemma~\ref{lemma:gaussian_example_lemma1} and Lemma~\ref{lemma:gaussian_example_lemma2} with Theorem~\ref{thm:combine_with_cheeger_simplified}.

\begin{proof}[Proof of Theorem~\ref{theorem:gaussian_example}]
We specify the ommited constants in the assumption of Theorem~\ref{theorem:gaussian_example}: we assume $\min_{i\ne j}\|{\mu_i-\mu_j}\|_2 \ge 25\sqrt{d}$, assume for any $x, x'\in\Real^d$ such that $\|{x}\|_2+ \|{x'}\|_2\le 2 \max_i\|{\mu_i}\|_2$ and $\|{x-x'}\|_2\ge \frac{1}{10} \min_{i\ne j}\|{\mu_i-\mu_j}\|_2$, there is $\augexample_t(x)\ne \augexample_t(x')$ for any $t\in[m]$.

Let $\Phi_{d}(z) = \Pr_{\xi\sim\mathcal{N}(0, I)} (\norm{\xi}_2\le z)$. Using the remark after Proposition 7.8 of ~\cite{massart2007concentration}, we can bound the tail probability for chi-square distribution as follows: for any $x>0$, there is $1-\Phi_{d}(\sqrt{d}+\sqrt{2x})\le \exp(-x)$. By Lemma~\ref{lemma:gaussian_example_lemma1}, we know $\alpha\le O(\exp(-4d))$.
	
	In Lemma~\ref{lemma:gaussian_example_lemma2}, set $\tau = \sigma$, we have for any $k'>r$, there is $\rho_{k'}\ge \Omega(c_\tau\cdot \exp(- \Phi_{d}^{-1}(\frac{2}{3})))$ where $c_\tau =  \min_{0 \le p \le 3/4} \frac{\Phi(\Phi^{-1}(p)+\tau)}{p} - 1 \ge \Omega(\tau) = \Omega(\sigma)$. 
	By concentration inequality, there must exists some universal constant $C>0$ such that for any $d\ge C$, there is $1-\Phi_{d}(\sqrt{\frac{3}{2}d}) \le \frac{1}{3}$. When this happens, we have $\Phi_d^{-1}(\frac{2}{3})\le \sqrt{\frac{3}{2}d}$, hence $\rho_{k'}\ge\Omega(\sigma \cdot \exp(-\sqrt{\frac{3}{2}d}))$. Since for $d\le C$ we can just treat $d$ as constant and still get the same bound, we have  $\rho_{k'}\ge\Omega(\sigma \cdot \exp(-\sqrt{\frac{3}{2}d}))$ for all $d\in\mathcal{Z}^+$.
	
	Set $k'=\lfloor k/2\rfloor$, we apply Theorem~\ref{thm:combine_with_cheeger_simplified} and get the bound we need.
\end{proof}


\subsection{Proof of Lemma~\ref{lemma:gaussian_example_lemma2}}\label{section:proof_of_gaussian_lemma2}
In this section we give a proof for Lemma~\ref{lemma:gaussian_example_lemma2}. We first introduce the following claim which states that for a given subset of augmented data, any two data close in $L_2$ norm cannot have very different chance of being augmented into this set.

\begin{claim}\label{claim:gaussian_example_claim1}
	In the setting of Theorem~\ref{theorem:gaussian_example}, given a set $S\subseteq \cup_{i\in[m]}\img_i$, where $\img_i$ is the image of $\augexample_i$. If $x\in \Real^d$ satisfies $\Pr(S|x) := \Pr_{\tilde{x}\sim\aug{x}} (\tilde{x}\in S) \ge\frac{2}{3}$. Then, for any $x'$ such that $\norm{x-x'}_2\le \tau$, there is 
	\begin{align*}
	\Pr(S|x') \ge \frac{1}{3}\cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right),
	\end{align*}
	where 
	\begin{align*}
	c_\sigma := \sigma \cdot  \Phi_d^{-1}(\frac{2}{3}),
	\end{align*}
	with $\Phi_{d}(z) := \Pr_{\xi\sim\mathcal{N}(0, I)} (\norm{\xi}_2\le z)$.
\end{claim}


\begin{proof}[Proof of Claim~\ref{claim:gaussian_example_claim1}]
	Given $x\in \Real^d$, define probability 
	\begin{align*}
	P_{\augexample}(S|x) := \Pr_{i \sim uni( [m])} \left(\augexample_i(x)\in S \right).
	\end{align*}
	By the definition of augmentation, we know 
	\begin{align*}
	\Pr(S|x) = \Exp{\xi\sim \mathcal{N}(0, \sigma^2I_{d\times d})}\left[P_h(S|x+\xi)\right].
	\end{align*}
	By the definition of $c_\sigma$, there is 
	\begin{align*}
	\Pr_{\xi\sim \mathcal{N}(0, \sigma^2I)} (\norm{\xi}_2\le c_\sigma)  = \frac{2}{3}.
	\end{align*}
	Since $\Pr(S|x)\ge \frac{2}{3}$ by assumption, we have 
	\begin{align*}
	\Exp{\xi\sim \mathcal{N}(0, \sigma^2I)} \left[P_h(S|x+\xi) \cdot \id{\norm{\xi}_2\le c_\sigma}\right] \ge \frac{1}{3}.
	\end{align*}
	Now we can bound the quanity of our interest:
	\begin{align*}
	\Pr(S|x') &= \frac{1}{(2\pi \sigma^2)^{d/2}}\int_{\xi} e^{-\frac{\norm{\xi}_2^2}{2\sigma^2}} P_h(S|x'+\xi)d\xi\\
	&= \frac{1}{(2\pi \sigma^2)^{d/2}} \int_{\xi} e^{-\frac{\norm{\xi + x - x'}_2^2}{2\sigma^2}} P_h(S|x+\xi)d\xi\\
	&\ge \frac{1}{(2\pi \sigma^2)^{d/2}}\int_{\xi} e^{-\frac{\norm{\xi + x - x'}_2^2}{2\sigma^2}} P_h(S|x+\xi) \cdot \id{\norm{\xi}_2\le c_\sigma}d\xi\\
	&\ge \frac{1}{(2\pi \sigma^2)^{d/2}} \int_{\xi} e^{-\frac{2c_\sigma\tau+\tau^2 + \norm{\xi}_2^2}{2\sigma^2}} P_h(S|x+\xi) \cdot \id{\norm{\xi}_2\le c_\sigma}d\xi\\
	&= e^{-\frac{2c_\sigma\tau + \tau^2}{2\sigma^2}} \cdot  \Exp{\xi\sim \mathcal{N}(0, \sigma^2I_{d\times d})} \left[P_h(S|x+\xi) \cdot \id{\norm{\xi}_2\le c_\sigma}\right]\\
	&\ge \frac{1}{3}\cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right).
	\end{align*}	
\end{proof}

We now give the proof of Lemma~\ref{lemma:gaussian_example_lemma2}.

\begin{proof}[Proof of Lemma~\ref{lemma:gaussian_example_lemma2}]
	Let $S_1, \cdots, S_{k'}$ be the disjoint sets that gives $\rho_{k'}$ in Definition~\ref{definition:multi_way_expansion_constant}.	First we notice that when $k'>r$, there must exist $t\in[k']$ such that for all $i\in[r]$, there is
	\begin{align}\label{equation:less_than_half}
	\Pr_{x\sim \mathcal{N}(\mu_i, I_{d\times d}), \tilde{x}\sim \aug{x}}(\tilde{x}\in S_t)\le\frac{1}{2}.
	\end{align}
	WLOG, we assume $t=1$. So we know that 
	\begin{align}\label{equation:rho_g_lower_bound}
	\rho_{k'} &= \max_{i\in[k']} \phi_G(S_i) 
	\ge \phi_G(S_1) 
	\ge \min_{j\in[r]} \frac{\Exp{x\sim \mathcal{N}(\mu_j, I_{d\times d})} \left[\Pr(S_1|x)(1-\Pr(S_1|x))\right]}{\Exp{x\sim \mathcal{N}(\mu_j, I_{d\times d})}\left[\Pr(S_1|x)\right]},
	\end{align}
	where \begin{align*}
	\Pr(S|x) := \Pr_{\tilde{x}\sim\aug{x}} (\tilde{x}\in S).
	\end{align*}
	WLOG, we assume $j=1$ minimizes the RHS of Equation~\eqref{equation:rho_g_lower_bound}, so we only need to prove
	\begin{align*}
	\frac{\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})} \left[\Pr(S_1|x)(1-\Pr(S_1|x))\right]}{\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})}\left[\Pr(S_1|x)\right]} \ge \frac{c_\tau}{18} \cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right).
	\end{align*} 
	
	We define the following set 
	\begin{align*}
	Q := \left\{x \bigg\vert  \Pr(S_1|x) \ge \frac{2}{3}\right\}.
	\end{align*}
	Let $P_1(x)$ be the PDF of distribution $\mathcal{N}(\mu_1, I)$. Notice that 
	\begin{align}\label{equation:at_least_one_true}
	\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})}\left[\Pr(S_1|x)\right] &= \int_x P_1(x) \Pr(S_1|x) dx\nonumber\\
	&= \int_{x\in Q} P_1(x) \Pr(S_1|x) dx + \int_{x\notin Q} P_1(x) \Pr(S_1|x) dx.
	\end{align}
	We can consider the following two cases.
	
	\textbf{Case 1:} $\int_{x\notin Q} P_1(x) \Pr(S_1|x) dx \ge \frac{1}{2}\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})}\left[\Pr(S_1|x)\right]$.
	
	This is the easy case because we have 
	\begin{align*}
	\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})} \left[\Pr(S_1|x)(1-\Pr(S_1|x))\right] &\ge \int_{x\notin Q} P_1(x) \Pr(S_1|x) (1-\Pr(S_1|x))dx\\
	&\ge \frac{1}{3}\int_{x\notin Q} P_1(x) \Pr(S_1|x) dx\\
	&\ge \frac{1}{6}\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})}\left[\Pr(S_1|x)\right].
	\end{align*}
	
	\textbf{Case 2:} $\int_{x\in Q} P_1(x) \Pr(S_1|x) dx \ge \frac{1}{2}\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})}\left[\Pr(S_1|x)\right]$.
	
	Define neighbourhood of $Q$ as \begin{align*}
	N(Q) := \left\{x \bigg \vert \norm{x-a}_2 \le \tau \text{ for some } a\in Q\right\}.
	\end{align*}
	We have 
	\begin{align*}
	\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})} \left[\Pr(S_1|x)(1-\Pr(S_1|x))\right] &\ge \int_{x\in N(Q)\backslash Q} P_1(x) \Pr(S_1|x) (1-\Pr(S_1|x))dx\\
	&\ge \frac{1}{9} \cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right)\cdot  \int_{x\in N(Q)\backslash Q}P_1(x) dx,
	\end{align*}
	where the second inequality is by Claim~\ref{claim:gaussian_example_claim1}. Notice that 
	\begin{align*}
	\int_{x\in Q} P_1(x)dx \le \frac{3}{2}\int_{x\in Q} P_1(x) \Pr(S_1|x)dx \le \frac{3}{2}\int_{x} P_1(x) \Pr(S_1|x)dx \le \frac{3}{4},
	\end{align*}
	where we use Equation~\eqref{equation:less_than_half}.
	According to the Gaussian isoperimetric inequality, there is  
	\begin{align*}
	\int_{x\in N(Q)\backslash Q}P_1(x) dx \ge c_\tau \int_{x\in Q} P_1(x)dx,
	\end{align*}
	where 
	\begin{align*}
	c_\tau   := \min_{0 \le p \le 3/4} \frac{\Phi(\Phi^{-1}(p)+\tau)}{p} - 1,
	\end{align*}
	with $\Phi(\cdot)$ being the function defined as
	\begin{align*}
	\Phi(z) := \int_{-\infty}^z  \frac{e^{-u^2/2}}{\sqrt{2\pi}}du.
	\end{align*}
	
	So we have 
	\begin{align*}
	\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})} \left[\Pr(S_1|x)(1-\Pr(S_1|x))\right] &\ge \frac{c_\tau}{9} \cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right)\cdot  \int_{x\in Q}P_1(x) dx\\
	&\ge \frac{c_\tau}{9} \cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right)\cdot  \int_{x\in Q}P_1(x) \Pr(S_1|x) dx\\
	&\ge \frac{c_\tau}{18} \cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right)\cdot  \Exp{x\sim \mathcal{N}(\mu_1, I)}\left[\Pr(S_1|x)\right].
	\end{align*}
	
	By Equation~\eqref{equation:at_least_one_true}, either case 1 or case 2 holds.
	Combining case 1 and case 2, we have 
	\begin{align*}
	\frac{\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})} \left[\Pr(S_1|x)(1-\Pr(S_1|x))\right]}{\Exp{x\sim \mathcal{N}(\mu_1, I_{d\times d})}\left[\Pr(S_1|x)\right]} &\ge \min\left\{\frac{1}{6}, \frac{c_\tau}{18} \cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right)\right\}\\
	&= \frac{c_\tau}{18} \cdot  \exp\left(-\frac{2c_\sigma\tau+\tau^2}{2\sigma^2}\right).
	\end{align*}
	
\end{proof}
